Enabling Uncertainty Estimation in Iterative Neural Networks

Turning pass-through network architectures into iterative ones, which use their own output as input, is a well-known approach for boosting performance. In this paper, we argue that such architectures offer an additional benefit: The convergence rate of their successive outputs is highly correlated with the accuracy of the value to which they converge. Thus, we can use the convergence rate as a useful proxy for uncertainty. This results in an approach to uncertainty estimation that provides state-of-the-art estimates at a much lower computational cost than techniques like Ensembles, and without requiring any modifications to the original iterative model. We demonstrate its practical value by embedding it in two application domains: road detection in aerial images and the estimation of aerodynamic properties of 2D and 3D shapes.

==> bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> bib/report.tex <==
\usepackage{named}

\usepackage{geometry}
\usepackage{times}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm,amssymb}
\usepackage{color}

\geometry{
 a4paper,
 left=21mm,
 right=21mm,
 top=16mm,
 bottom=16mm,
 }
 
%\setlength{\oddsidemargin}{0.0in}
%\setlength{\topmargin}{-0.125in}
%\setlength{\textwidth}{6.25in}
%\setlength{\textheight}{8.75in}
%\parskip 6pt plus 3pt minus 2pt

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\im}{\item}
\newcommand{\comment}[1]{}
\newcommand{\missing}[1]{\begin{large} {\bf ADD:} {\em #1} \end{large}}
\newcommand{\note}[1]{\begin{center} \noindent\framebox{\begin{minipage}{8cm}{\bf #1}\end{minipage}}\end{center}\\}
\newcommand{\rmk}[1]{{\color{red}{ \bf #1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\url}[1]{#1}

\newif\ifsubmit
\submitfalse

\newif\ifdraft
\draftfalse

\newcommand{\dspace}{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\newcommand{\sspace}{\renewcommand{\baselinestretch}{1.0}\large\normalsize}
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SubSection}[1]{\subsection{#1}}
\sspace

\renewcommand{\floatpagefraction}{1.0}


==> fig/airfoils.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[htb]
    \centering
    \begin{tabular}{cc}
        \hspace{-2mm}\includegraphics[width=0.49\textwidth]{images/airfoil_accuracy.pdf}&
        \hspace{-2mm}\includegraphics[width=0.49\textwidth]{images/airfoil_optimization.pdf}\\
        (a) & (b)
    \end{tabular}   
    \vspace{-3mm} 
    \caption{\small 
        \textbf{Airfoils.} (a) Accuracy of the lift-to-drag estimate as a function of the number of exemplars used to train the emulators. (b) Lift-to-drag ratio of the shapes during optimization, as a function of number of iterations. \PF{Could you something visual? And change the labels to conform to those in the text.}}
    \label{fig:airfoils}
\end{figure*}
    
    
    

==> fig/airfoils_imp.tex <==
\begin{figure*}[htb]
    \centering
    \begin{tabular}{cc}
        \hspace{-2mm}\includegraphics[width=0.49\textwidth]{images/improved_l2d.pdf}&
        \hspace{-2mm}\includegraphics[width=0.49\textwidth]{images/improved_pressure.pdf}\\
    \end{tabular}     
    \caption{\small 
        \textbf{Iterations improve performance.}
        Result for airfoils emulator predictions accuracy for lift-to-drag and pressure predictions. Several consecutives iteration demonstrate increasing quality of estimations.
        }
    \label{fig:airfoils_imp}
\end{figure*}
    
    
    

==> fig/bo.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US
\clearpage
\begin{figure*}[!t]
    \includegraphics[width=\textwidth]{images/bo_example.pdf}
    % \vspace{-8mm}
    \centering
    \caption{\small 
    \textbf{Bayesian Optimization.} Given three initial data points for the function (dashed blue), we want to optimize,  we train a GP surrogate model (Step 1) and compute the UCB acquisition function~\citep{Auer02} over the $[0, 1]$  range (Steps 2-3). We then select the points that maximize, evaluate the target function at those points, and include the results in our training dataset (Step 4). The process is then iterated and, eventually, we find the true maximum of the function at $x \approx 1$, whereas a simple gradient based method would probably have remained trapped at the local maximum $x \approx 0.58$. }
    % \vspace{-2mm}
    \label{fig:bo_example}
\end{figure*}

==> fig/cars.tex <==
\begin{figure*}[htb]
    \centering
    \begin{tabular}{cc}
        \hspace{-2mm}\includegraphics[width=0.49\textwidth]{images/cars_accuracy.pdf}&
        \hspace{-2mm}\includegraphics[width=0.49\textwidth]{images/cars_optimization.pdf}\\
    \end{tabular}     
    \caption{\small 
        \textbf{Cars results.}
        Result for emulator predictions accuracy and shape optimization for cars dataset.
        }
    \label{fig:cars}
\end{figure*}
    
    
    

==> fig/emulator.tex <==
\begin{figure*}[htb]
    \includegraphics[width=\textwidth]{images/gnn_emulator.pdf}
    \vspace{-4mm}
    \centering
    \caption{\small 
    \textbf{GNN emulator:}
    Given an input mesh of an airfoil, emulator iteratively produces a sequence of pressure and lift-to-drag predictions, following similar setup as original simulator.
    }
    \label{fig:emulator}
\end{figure*}




==> fig/interpol_div.tex <==
\begin{figure*}[htb]
    \begin{tabular}{cc}
       \includegraphics[width=0.45\textwidth]{images/toy_pred.pdf}& \includegraphics[width=0.45\textwidth]{images/toy_pred_1.pdf}\\
       \includegraphics[width=0.45\textwidth]{images/toy_pred_2.pdf}& \includegraphics[width=0.45\textwidth]{images/toy_pred_20.pdf}\\
    \end{tabular}
        \vspace{-3mm}
        \centering
        \caption{\small 
        \textbf{Convergence for various inputs.} Following experiments in Fig.~\ref{fig:interpol1} and Fig.~\ref{fig:interpol2}, we trained an MLP model on data covering the range $[-1, 3]$ for $x$ and $y = 1.5x^{3} - 5x^{2} + x$. Using our reentrant procedure, we made predictions for three points: $x = 1$, $x = 4$, and $x = 20$. Convergence was nearly instant for $x=1$, took more iterations for $x=4$, and surprisingly, we observed oscillations rather than convergence for $x=20$.}
        
        % Similar to the experiments in Fig.~\ref{fig:interpol1} and Fig.~\ref{fig:interpol2}, we have trained an MLP model on data that was consists of $x$ in the range $[-1, 3]$ and $y = 1.5x^{3} - 5x^{2} + x$. We have applied our reentrant procedure to produce predictions for three points $x = 1, x = 4, $ and $x = 20$. As it can be seen, for $x=1$, as it is an in-distribution point, model converges almost instantly. For more remote point $x=4$, convergence happens though it takes more iterations. Interestingly, but for $x=20$, we observe that the prediction do not converge but oscillate instead.
        % }
        \label{fig:interpol3}
    \end{figure*}
    


==> fig/iter_refinement_mos.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


% \begin{figure}[htb]
%     \includegraphics[width=0.49\textwidth]{images/refinement.png}
%     \vspace{-5mm}
%     \centering
%     \caption{\small 
%     \textbf{Iterative refinement.} The model iteratively applies the same U-Net f to produce progressive refinements of the predicted delineation. The final loss is a weighted sum of partial losses computed at the end of each step. The original $\by_{0}$ input is considered to be empty and therefore is initialized with $\bzer$.}
%     \label{fig:mosRefinement}
% \end{figure}

\begin{figure}[htb]
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.47\textwidth]{images/refinement.png} \\
        \includegraphics[width=0.47\textwidth]{images/refinement_qualitative.png}\\
    \end{tabular}  
    % \vspace{-7mm}   
    \caption{\small \textbf{Iterative refinement from~\cite{Mosinska18}.} \textbf{(Top):} The model iteratively applies the same U-Net to progressively refine a binary mask of road pixels. The final loss is a weighted sum of partial losses computed at the end of each step. The original $\by_{0}$ input is considered to be empty and therefore is initialized with $\bzer$. \textbf{(Bottom):} Prediction after 1, 2 and 3 refinement iterations. The right-most image is the ground-truth. The red boxes highlight parts of the image where refinement is closing gaps. }        % \vspace{-2mm} 
    \label{fig:mosRefinement}
\end{figure}



==> fig/l_int.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table*}[ht!]
    \centering
    \begin{tabular}{c|cccc|c} 
    &  \#1: w/o pressure &  \#2: w/ pressure &  \#3: integration &  \#4:  \textit{Reentrant} & \\
    \hline
    AIR & $3.309 \pm 0.01$ &  $2.807 \pm 0.01$ & $3.61 \pm 0.01$ & \textbf{\textcolor{gray}{2.6}} $\pm$ \textbf{\textcolor{gray}{0.01}} & \\ 
    \hline
    CARS & $0.35 \pm 0.02$ & 0.32 $\pm$ 0.01 & 0.51 $\pm$ 0.07 & \textbf{\textcolor{gray}{0.30}} $\pm$ \textbf{\textcolor{gray}{0.01}} & \\ 
    
    \end{tabular}
    \vspace{-2mm}
    \caption{\small {\bf Mean error and variance of  predicted performance} for the four methods of Section~\ref{app:integration}.}
    \label{tab:l_int}  
\end{table*}



==> fig/opt_cars.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\begin{figure}[htb]
    \includegraphics[width=0.49\textwidth]{images/optimized_cars.png}
    \vspace{-5mm}
    \centering
    \caption{\small 
    \textbf{Optimized car shapes.} {\bf Left.} A car from the initial training set. {\bf Right.} Best final car. The color depict the vector $\by$ of pressure values predicted by the emulator.}
    \label{fig:optimCar}
\end{figure}



==> fig/propagation.tex <==
\begin{figure*}[htb]
    \includegraphics[width=0.9\textwidth]{images/propagation.pdf}
    % \vspace{-4mm}
    \centering
    \caption{\small 
    \textbf{Information propagation:}
    With each iteration information used to make prediction in one particular point is collected from broader set of neighbours.
    }
    \label{fig:simulator}
\end{figure*}




==> fig/sim_unc.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[htb]
    \includegraphics[width=\textwidth]{images/conv.pdf}
    \vspace{-7mm}
    \centering
    \caption{\small 
    \textbf{Simulator convergence.}  (Simple Shape) Convergence occurs after only 6 iterations, (Complex shape) For this more complex shape, 40 iterations are needed.  This motivates us to threat number of iterations until convergence as confidence measure.}
    \label{fig:conv}
\end{figure*}



==> fig/simulator.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[htb]
\centering
\begin{tabular}{cc}
    \hspace{-2mm}\includegraphics[width=0.49\textwidth]{images/simulations.pdf}&
    \hspace{-2mm}\includegraphics[width=0.49\textwidth]{images/gnn_emulator.pdf}\\[1mm]
    Simulator & Reentrant GNN
\end{tabular}    
\vspace{-4mm}
\caption{\small 
    \textbf{From simulator to reentrant GNN.} {\bf (Simulator)} Consider distant airfoil locations 1 and 2. In a traditional simulator, results at location 1 can easily influence the results at location 2 in spite of their distance, as often happens in real life. {\bf  (Reentrant GNN) }The recursive nature of the computation makes it possible to take into account all the physical parameter values while estimating one at a specific location, hence making the interaction between distant locations straightforward.}
\label{fig:simulator}
\end{figure*}




==> fig/train_inference.tex <==

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{minipage}{0.49\textwidth}
    \begin{algorithm}[H]
        \centering
        \caption{\sbo{} Training}\label{algorithm}
        \begin{algorithmic}[1]
            \Require Emulator $\widetilde{g}_{\Theta}$, epochs $N$, learning rate $\alpha$, dataset $D$, loss weight $\gamma$, max iterations $M$.
            \Ensure Trained $\widetilde{g}_{\Theta}

            \For{\texttt{i in 1...N}}
            \State \texttt{$\bx, \by, r \sim D$}
            \State \texttt{$\tilde{\by} = \textbf{0}$} \Comment{Initialize with zeros}
                \For{\texttt{j in 1...M}}
                    \State \texttt{$\tilde{\by}, \tilde{r} = \widetilde{g}_{\Theta}(\bx, \tilde{\by})$}
                \EndFor
            \State \texttt{$l = \|r-\tilde{r}\| + \gamma\|\by - \tilde{\by}\|$}
            \State \Theta \leftarrow \Theta - \alpha \nabla_{\Theta} l

            \EndFor
            
        \end{algorithmic}
    \end{algorithm}
    \end{minipage}
    \hfill
    \begin{minipage}{0.46\textwidth}
    \begin{algorithm}[H]
        \centering
        \caption{\sbo{} Inference}\label{algorithm1}
        \begin{algorithmic}[1]
            \Require Emulator $\widetilde{g}_{\Theta}$, mesh $\bx$, iterations $M$
            \Ensure physical attributes $\tilde{\by}, \tilde{r}$
            
            \State \texttt{$\tilde{\by}^{0} = \textbf{0}$} 
            \For{\texttt{j in 1...M}}
            \State \texttt{$\tilde{\by}^{j}, \tilde{r}^{j} = \widetilde{g}_{\Theta}(\bx, \tilde{\by}^{j-1})$}
            \EndFor
            \State \ND{Describe uncertainty here}

            % \Return asdfasdf
        \end{algorithmic}
    \end{algorithm}
    \end{minipage}
